IICNet: A Generic Framework for Reversible Image Conversion

Reversible image conversion (RIC) aims to build a reversible transformation between specific visual content (e.g., short videos) and an embedding image, where the original content can be restored from the embedding when necessary. This work develops Invertible Image Conversion Net (IICNet) as a generic solution to various RIC tasks due to its strong capacity and task-independent design. Unlike previous encoder-decoder based methods, IICNet maintains a highly invertible structure based on invertible neural networks (INNs) to better preserve the information during conversion. We use a relation module and a channel squeeze layer to improve the INN nonlinearity to extract cross-image relations and the network flexibility, respectively. Experimental results demonstrate that IICNet outperforms the specifically-designed methods on existing RIC tasks and can generalize well to various newly-explored tasks. With our generic IICNet, we no longer need to hand-engineer task-specific embedding networks for rapidly occurring visual content. Our source codes are available at: https://github.com/felixcheng97/IICNet.

==> IICNet_ A Generic Framework for Invertible Image Conversion Camera Ready/tex/conclusion.tex <==
We present a generic framework IICNet for various Reversible Image Conversion (RIC) tasks. IICNet maintains a task-independent and highly invertible architecture based on invertible neural networks (INNs), which largely mitigates the information loss problem. Due to strict invertibility, INNs have limitations in terms of dimensional flexibility and non-linear representation capacity. Our proposed Relation Module and Channel Squeeze Layer can greatly alleviate such limitations and preserve the information-reserving ability of INNs, promisingly applicable to other INNs applications.
IICNet yields state-of-the-art performance on some studied RIC tasks, such as Spatial-Temporal Video Embedding and Mononizing Binocular Images. We also extend to some unexplored tasks and the stenography task to further show the generalization of our IICNet. We hope the generalization and high performance of the proposed framework could help in more practical applications.


==> IICNet_ A Generic Framework for Invertible Image Conversion Camera Ready/tex/experiments.tex <==
\begin{figure}
    \begin{subfigure}{1.0\linewidth}
        \includegraphics[width=0.98\linewidth]{figures/video-embedding.pdf}
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{1.0\linewidth}
        \begin{subfigure}{0.495\linewidth}\hfil Zhu et al.~\cite{zhu-2020-video}\end{subfigure}
        \begin{subfigure}{0.495\linewidth}\hfil Ours\end{subfigure}
	\end{subfigure}
	\caption{Visual result comparisons on embedding images.}
	\label{fig:task1-embedding}
\end{figure}

\begin{figure*}
    \begin{subfigure}{0.02\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Zhu et al.~\cite{zhu-2020-video}}}} \\
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}} \\
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{1\linewidth}
            \includegraphics[width=1\linewidth]{figures/video-restore.pdf}
        \end{subfigure}
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.02\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 1\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 3\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 5 (ref.)\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 7\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 9\end{subfigure}
    \end{subfigure}
    \caption{Visual result comparisons on restored frames.}
	\label{fig:task1-restore}
\end{figure*}

This section first reports experiments conducted on previously-studied RIC tasks in Section~\ref{spatial-temporal-video-embedding} and~\ref{mononizing-binocular-images}, followed by the results of some newly-explored tasks in Section~\ref{dual-view-images} and~\ref{composition-and-decomposition-images}. In Section~\ref{hiding-images-in-an-image}, we also try the steganography task of hiding several images in one cover image. Please check out our supplementary materials for experimental setting details.

\subsection{Spatial-Temporal Video Embedding}
\label{spatial-temporal-video-embedding}

Video Snapshot~\cite{zhu-2020-video} aims to embed a sequence of video frames into one embedding image with the same resolution, which can be converted back to the original video sequence. Our proposed IICNet not only performs better but can even extend to embed the video frames spatiotemporally into a lower-resolution embedding image. 

\textbf{Dataset and Processing.} We use the high-quality DAVIS $2017$ video dataset~\cite{Jordi2017DAVIS} in this task. We use the official TrainVal set plus half of the Test-Dev set as the train set, another half of the Test-Dev set as the validation set, and the Test-Challenge set as the test set. To make our model more robust on different motion levels of video inputs, for each video sample in the train set, we subsample all the possible video subsamples with a time step of $5$ between consecutive frames, where we select the middle frame as the reference image.

\textbf{Result Comparison.} We only report the comparison results on the test set with embedding range $N = 9$, since Video Snapshot~\cite{zhu-2020-video} only provides the pre-trained model for this level of embedding range. We study on the performance at different time step levels of $1$, $3$, $5$ to test models' capacity in handling large motions. Statistics in Table~\ref{tab:task1-comparison} shows that our method significantly outperforms the baseline method at all time step levels by a large margin. Without dependence on optical flow, our method has less performance drop as the time step grows. We also offer grayscale PSNR and SSIM comparison in our supplemental materials for reference.

Figure~\ref{fig:task1-embedding} and Figure~\ref{fig:task1-restore} show the visualization results of the embedding images and the restored frames, respectively. Evident artifacts are found in the results of the baseline method, especially for the embedding image. In contrast, our embedding and restored images contain very few artifacts, demonstrating the effectiveness of the employed INN architecture in RIC tasks.

\begin{table}
  \begin{center}
    \begin{tabular}{p{29pt}|p{39pt}p{35pt}p{39pt}p{35pt}}
      \toprule[1pt]
      \multirow{2}{29pt}{\centering\textbf{Range}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 5 & \hfil 39.033 & \hfil 0.9539 & \hfil 41.836 & \hfil 0.9810 \\
      \hfil 7 & \hfil 38.336 & \hfil 0.9463 & \hfil 39.010 & \hfil 0.9674 \\
      \hfil 9 & \hfil 37.750 & \hfil 0.9419 & \hfil 36.866 & \hfil 0.9532 \\
      \hline\Tstrut
      \hfil 3 ($\bm{\times}$2) & \hfil 37.763 & \hfil 0.9608 & \hfil 36.891 & \hfil 0.9547 \\
      \hfil 5 ($\bm{\times}$2) & \hfil 36.622 & \hfil 0.9482 & \hfil 34.272 & \hfil 0.9242 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Results on Spatial-Temporal Video Embedding test set with different embedding ranges and resolutions.}
  \label{tab:task1-range}
\end{table}

\textbf{Embedding Range.} To investigate the embedding capacity of our method, we conduct experiments using different embedding ranges ($5, 7, 9$ input images). Similarly, we subsample the training videos with a time step of $5$, and test at a time step level of $1$. Intuitively, more input images indicate a more challenging task, where there is more motion information to be embedded into the embedding image. From Table~\ref{tab:task1-range}, we can see that our method outperforms the previous method at all levels of the embedding range and has less performance drop as the embedding range increases. 

\begin{figure*}[ht!]
    \begin{subfigure}{0.02\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][3.7cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{L. Bino-View}}} \\
        \parbox[][3.7cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{R. Bino-View}}}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \includegraphics[width=1\linewidth]{figures/mono.pdf}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.02\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{0.256\linewidth}\hfil GT\end{subfigure}
        \begin{subfigure}{0.372\linewidth}\hfil Hu et al.~\cite{hu-2020-mononizing}\end{subfigure}
        \begin{subfigure}{0.372\linewidth}\hfil Ours\end{subfigure}
    \end{subfigure}
	\caption{Visual comparison results of the restored Binocular Images. We show the zoomed-in patches with the corresponding error map aside. Note that we amplified the error maps by 10 times for better visualization.}
	\label{fig:task2-comparison}
\end{figure*}

\textbf{Spatial-Temporal Embedding.} We further show the experimental results of our method to embed the input video sequence spatially and temporally into a lower-resolution embedding image. To the best of our knowledge, no previous work can do the spatial-temporal embedding task. We report the results of embedding $N = 3, 5$ into a $2$ times lower resolution in Table~\ref{tab:task1-range}. They are both conducted with a time step of $5$ and $1$ for training and testing, respectively. We can see that even we compress the input frames up to $20$ times smaller, still the model can have a good preview image and restored frames.

\textbf{Ablation Studies.} To validate the effectiveness of the components in our network and the utilization of the frequency loss, we report some ablation studies with embedding range of $5$ and a time step of $1$ in Table~\ref{tab:ablation}. From the experiments, we find the frequency loss greatly contributes to the artifacts-free embedding. Also, the proposed non-linear Relation Module works well to integrate the cross-image relationship and boost the performance.

\begin{table}
  \begin{center}
    \begin{tabular}{p{58pt}|p{29pt}p{29pt}p{29pt}p{29pt}}
      \toprule[1pt]
      \multirow{2}{58pt}{\centering\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil Ours w/o Fre. & \hfil 33.063 & \hfil 0.858 & \hfil 41.841 & \hfil 0.982 \\
      \hfil Ours w/o Rel. & \hfil 38.617 & \hfil 0.952 & \hfil 40.386 & \hfil 0.976 \\
      \hfil Ours & \hfil 39.033 & \hfil 0.954 & \hfil 41.836 & \hfil 0.981 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Ablation studies of frequency loss and Relation Module.}
  \label{tab:ablation}
\end{table}

\begin{table}[h!]
  \begin{center}
    \begin{tabular}{p{20pt}|p{56pt}|p{56pt}|p{56pt}}
      \toprule[1pt]
      \multirow{2}{20pt}{\ } & \multicolumn{1}{c|}{\textbf{Mono-view}} & \multicolumn{1}{c|}{\textbf{L. Bino-view}} & \multicolumn{1}{c}{\textbf{R. Bino-view}} \\ 
    %   \cline{2-5} & \hfil Snapshot & \hfil Ours & \hfil Snapshot & \hfil Ours \\
      \ & \hfil PSNR \text{  } SSIM& \hfil PSNR \text{  } SSIM & \hfil PSNR \text{  } SSIM \\
      \hline\Tstrut
      \hfil \cite{46526} & \hfil 26.1\ \ \ \ \ \ 0.81 & \hfil -\ \ \ \ \ \ \ \ \ \ \ \ - & \hfil 27.9\ \ \ \ \ \ 0.88 \\
      \hfil \cite{xia-2018-invertible} & \hfil 28.0\ \ \ \ \ \ 0.89 & \hfil 28.7\ \ \ \ \ \ 0.92 & \hfil 30.7\ \ \ \ \ \ 0.92 \\
      \hfil \cite{hu-2020-mononizing}  & \hfil 37.8\ \ \ \ \ \ \textbf{0.97} & \hfil 38.3\ \ \ \ \ \ 0.99 & \hfil 37.3\ \ \ \ \ \ 0.98 \\
      \hfil Ours & \hfil \textbf{37.9}\ \ \ \ \ \ 0.96 & \hfil \textbf{44.8}\ \ \ \ \ \ \textbf{0.99} & \hfil \textbf{39.4}\ \ \ \ \ \ \textbf{0.99} \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Results on Mononizing Binocular Images test set.}
  \label{tab:task2-comparison}
\end{table}

\subsection{Mononizing Binocular Images}
\label{mononizing-binocular-images}
We also experiment on another studied Mononizing Binocular Images task~\cite{hu-2020-mononizing}, which aims to convert binocular images or videos into monocular ones with the stereo information implicitly encoded. In this way, monocular devices can cope with stereoscopic data, and the original stereo content can be restored when necessary. We demonstrate that our framework outperforms state-of-the-art methods. 

Same as~\cite{hu-2020-mononizing}, we train on Flickr1024 dataset~\cite{Flickr1024} with the official train and test splits. Quantitative results are shown in Table~\ref{tab:task2-comparison}. We achieve the best performance especially for the restored images, with improvement of $6.5$dB for the left-views and $2.1$dB for the right-views. Although Mono3D already achieves good performance, still we can see some structural artifacts like the street lamp and the electric tower in the zoomed-in restored patches, as shown in Figure~\ref{fig:task2-comparison}, while our method can restore nearly artifact-free binocular-views. Although we only train our network on image dataset, when applying to video in a per-frame manner, the results show strong temporal consistency. Some demos can be found in supplementary materials.

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_normal.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_zoom.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_normal.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_zoom.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.32\linewidth}\hfil Embedding\end{subfigure}
        \begin{subfigure}{0.32\linewidth}\hfil Normal-View\end{subfigure}
        \begin{subfigure}{0.32\linewidth}\hfil Zoomed-View\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Embedding Dual-View Images.}
	\label{fig:application1-visual}
\end{figure}

\begin{table}
  \begin{center}
    \begin{tabular}{p{35pt}|p{50pt}p{50pt}p{50pt}}
      \toprule[1pt]
      \hfil \textbf{Modes} & \hfil \textbf{Embedding} & \hfil \textbf{Normal} & \hfil \textbf{Zoomed} \\
      \hline\Tstrut
      \hfil $\times$ 2 & \hfil 38.541 & \hfil 50.277 & \hfil 43.806  \\
      \hfil $\times$ 4 & \hfil 38.271 & \hfil 48.740 & \hfil 43.694  \\
      \hfil $\times$ 8 & \hfil 38.607 & \hfil 48.923 & \hfil 43.610  \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Embedding Dual-View Images.}
  \label{tab:application1-psnr}
\end{table}


\subsection{Embedding Dual-View Images}
\label{dual-view-images}
Dual-View Camera Mode is an advanced technology in the field of smartphone cameras, which is first available on HUAWEI P30 Pro~\cite{dual_view}. Users can record split-screen images or videos with the primary camera capturing normal-view images or videos on the left and the zoom lens capturing zoomed-view ($\times 4$) images or videos on the right. 

Similar to binocular images, not all devices support dual-view images, where our method can serve as a backward-compatible solution by embedding the dual-view images into one normal-view image. We train and test our method using pairs of zoomed-view ($\times 2$,$\times 4$,$\times 8$) and normal-view images generated from the DIV2K dataset~\cite{Agustsson_2017_CVPR_Workshops}, with normal-view images as reference images. Detailed settings can be found in the supplementary materials.

Quantitative results in Table~\ref{tab:application1-psnr} show that our method achieves great performance to embed dual-view images in terms of both PSNR and SSIM. We also show some visual results in Figure~\ref{fig:application1-visual}, where we can see that both the embedding and restored images are nearly perfect. 

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_fg.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_bg.jpeg}
		\end{subfigure}
	\end{subfigure}
	\\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_embedding.jpeg}
    	\end{subfigure}%
    	\begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_fg.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_bg.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.24\linewidth}\hfil Embedding\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Composed\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Foreground\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Background\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Composition and Decomposition.}
	\label{fig:application2-visual}
\end{figure}

\begin{table}
  \begin{center}
    \begin{tabular}{p{27pt}|p{38pt}p{38pt}p{38pt}p{38pt}}
      \toprule[1pt]
      \hfil \textbf{Task} & \hfil \textbf{Embed.} & \hfil \textbf{Comp.} &  \hfil \textbf{Fg.} & \hfil \textbf{Bg.} \\
      \hline\Tstrut
      \hfil Adobe & \hfil 45.638 & \hfil 52.672 & \hfil 45.120 & \hfil 45.071 \\
      \hfil Real & \hfil 46.757 & \hfil 58.324 & \hfil - & \hfil 44.325  \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Composition and Decomposition.}
  \label{tab:application2-psnr}
\end{table}

\subsection{Composition and Decomposition}
\label{composition-and-decomposition-images}
Photoshop~\cite{photoshop} is a popular image editing software, where users can use multiple layers to perform tasks such as compositing multiple images into one. Usually, the composition process is not reversible, so we cannot recover the sheltered part of the background of the composed image. However, with our method, we can allow the ``composed image" to embed all the layer images. In this way, although we only store and transmit one ``composed image" as before, users can also get the original layers for further usage.

Since there is no publicly available dataset for composition and decomposition, we instead train and test our method on two Matting datasets: Adobe Deep Matting dataset~\cite{deep-image-matting} and Real Matting dataset~\cite{BMSengupta20}. Note that Real Matting dataset does not have ground truth for foreground. Details setting is available in supplementary materials.

Table~\ref{tab:application2-psnr} shows the quantitative performance of our method on the two datasets. We also include some visual results in Figure~\ref{fig:application2-visual}. We can see that our method performs well and is verified to be applicable to the task of composing and decomposing images.

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame1.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame2.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame3.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame4.jpeg}
    	\end{subfigure}%
	    \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame5.jpeg}
    	\end{subfigure}%
	\end{subfigure}
	\\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame1.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame2.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame3.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame4.jpeg}
    	\end{subfigure}%
	    \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame5.jpeg}
    	\end{subfigure}%
	\end{subfigure}
	\\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.155\linewidth}\hfil Embed.\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Cover\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 1\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 2\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 3\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 4\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Hiding Images in Image}
	\label{fig:application3-visual}
\end{figure}

\begin{table}
  \begin{center}
    % \renewcommand\tabcolsep{5.0pt}
    \begin{tabular}{p{41pt}|p{33pt}p{33pt}p{33pt}p{33pt}}
      \toprule[1pt]
      \multirow{2}{41pt}{\centering\textbf{\#\ Embed.}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 2 & \hfil 38.911 & \hfil 0.9482 & \hfil 49.384 & \hfil 0.9951 \\
      \hfil 3 & \hfil 37.320 & \hfil 0.9277 & \hfil 43.671 & \hfil 0.9854 \\
      \hfil 4 & \hfil 36.221 & \hfil 0.9115 & \hfil 39.802 & \hfil 0.9743 \\
      \hfil 5 & \hfil 36.110 & \hfil 0.9064 & \hfil 37.777 & \hfil 0.9629 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Hiding Images in an Image.}
  \label{tab:application3-psnr-ssim}
\end{table}

\subsection{Hiding Images in an Image}
\label{hiding-images-in-an-image}
To show the generality of our proposed model, we try the hardest task to hide several unrelated images with our model, which can be viewed as a kind of stenography. We obtain general images from the Flicker 2W dataset~\cite{liu2020unified}. We conduct experiments to embed $2$, $3$, $4$, $5$ images into one image, and the numerical results are listed in Table~\ref{tab:application3-psnr-ssim}. From the results, we can see that our method achieves relatively good performance even when embedding $5$ images into one, demonstrating the strong generality of our method. From the visual results shown in Figure~\ref{fig:application3-visual}, despite the variety of colors and structures of the images, we can restore them with no viewable artifacts.






==> IICNet_ A Generic Framework for Invertible Image Conversion Camera Ready/tex/introduction.tex <==
Visual media can be classified into different types, including live photos~\cite{live_photo}, binocular images or videos~\cite{hu-2020-mononizing}, and dual-view images or videos~\cite{dual_view}. On the one hand, specific devices or platforms are required to view this visual media content. For example, binocular content may only be applicable in 3D devices, so we may need to generate corresponding monocular content to make them compatible with common devices~\cite{hu-2020-mononizing}. Instead of simply dropping part of the original content, a better choice is to build a reversible transformation, where the embedding is compatible with most devices, and the original content can be restored when necessary. On the other hand, a reversible single embedding image can help save the cost of storage and transmission bandwidth. To address these challenges, several Reversible Image Conversion (RIC) tasks~\cite{hu-2020-mononizing,xia-2018-invertible,zhu-2020-video} have been studied, which establish reversible transformation between visual content and an embedding image. Some examples are shown in Figure~\ref{fig:front}.

RIC tasks are challenging since we often need to embed much richer information implicitly in one single image, which may lead to unavoidable information loss. Hence, one of the key objectives in RIC tasks is to mitigate such information loss. However, previous works~\cite{hu-2020-mononizing,xia-2018-invertible,zhu-2020-video} usually employ an encoder-decoder based framework, which learns the informative bottleneck representation but has limited ability to capture the lost information~\cite{wang2020modeling,xiao2020invertible}. For example, Video Snapshot~\cite{zhu-2020-video} embeds a video preview into a single image and restores the original content by cascaded encoders and decoders. Although they sacrifice the embedding quality to embed as much information as possible, the restored frames are still not highly accurate. Furthermore, with the rapid growth of media formats, there is an increasing interest in the RIC tasks. Although RIC tasks share the same embedding-restoration procedure and the goal of obtaining high-quality embedding and restored images, previous methods usually have task-specific designs, such as optical flow in Video Snapshot~\cite{zhu-2020-video} and hardly generalize to other types of visual content. It is desirable to develop a general framework so that a generic framework can be adapted to all types of RIC tasks.

Considering these aspects, we propose Invertible Image Conversion Net (IICNet) as a generic framework for RIC tasks. To alleviate the information loss problem, we utilize invertible neural networks (INNs)~\cite{dinh2015nice,dinh2017density} as a strictly invertible embedding module. A Channel Squeeze Layer is also proposed to be incorporated into INNs for dimensional reduction while only minor deviation is introduced to the invertible architecture. Furthermore, to solve the problem that INNs contain limited non-linear transformation capacity~\cite{dinh2015nice}, we design a Relation Module to strengthen the non-linear representation capability that captures cross-image relation, in which the same-resolution transformation and residual connection help avoid extra information loss. These two new modules increase the flexibility and capacity of our network while keeping the advantage of INNs for reversibility. With strong embedding capacity and generic modules, IICNet does not rely on any task-specific technique as prior work, which makes it possible to deal with different content types. We also allow lower-resolution embedding for higher compression rates.

Here, we give a concrete example for illustration, as shown in Figure~\ref{fig:front}(a). Given a sequence of video frames, our IICNet can embed the spatial-temporal information of the sequence into one lower-resolution image that is visually similar to the downsampled middle reference frame.  There are some promising applications. First, we may embed a short video clip or live photo in one image. Second, we can embed a high-resolution high-FPS video into a low-resolution low-FPS video. In this way, we can allow flexible adoptions for different devices and save storage. Other potential applications are shown in Figure~\ref{fig:front}(b-e), including mononizing binocular images or videos, embedding dual-view images or multi-layer images, and even the general image hiding steganography task.

We conduct extensive experiments on five RIC tasks, in which our method outperforms other state-of-the-art methods by a large margin on all the studied tasks. Also, an ablation study is conducted for network modules and loss functions. Some detailed information and demo results are included in the supplementary materials. All the source codes and pre-trained models will be publicly available on Github. Our contributions are summarized as follows:
\begin{itemize}
    \item We present the first generic framework IICNet with the INN architecture that achieves state-of-the-art performance on five RIC tasks. IICNet allows various types of multimedia content to suit different devices and saves storage and bandwidth. 

    \item We propose a novel Channel Squeeze Layer and Relation Module incorporated into INNs to improve model flexibility and capacity while keeping the strength of reversibility.%, which can be extended to other applications with INNs.
    
    \item We study five practical RIC tasks, including two newly-explored ones, which are embedding a dual-view image into a single-view one and the reversible conversion between multi-layer images and a single image.

\end{itemize}

\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.5]{figures/overview.pdf}
\end{center}
\caption{Overview of the proposed network.}
\label{fig:overview}
\end{figure*}


==> IICNet_ A Generic Framework for Invertible Image Conversion Camera Ready/tex/method.tex <==
The proposed IICNet for general Reversible Image Conversion (RIC) tasks aims to encode a series of input images into one reversible image (embedding image), which can have either the same or lower resolution. The embedding image can be decoded back to the original inputs with the network backward passing. The key is to use invertible neural networks (INNs) to model such a bijective mapping. An overview of our generic framework is shown in Figure~\ref{fig:overview}. Specifically, IICNet sequentially contains a \textbf{Relation Module}, an \textbf{Invertible Embedding Module} (an optional Invertible Downscaling Module plus several Coupling Layers), a \textbf{Channel Squeeze Layer}, and a \textbf{Quantization Layer}.

\subsection{Model Formulation} \label{model-formulation}
Formally, the input of IICNet is a series of $N$ input RGB images $\{\bm{i}_n\}_{n=1}^N$ with $\bm{i}_n \in \mathbb{R}^{3 \times H \times W}$, where $H$ and $W$ are the height and width, respectively. IICNet can forwardly encode the input images into an embedding image $\bm{e} \in \mathbb{R}^{3 \times H' \times W'}$, with embedding height $H'$ and width $W'$, which is visually indistinguishable from the reference image $\bm{e}_{ref}$. IICNet can then backwardly decode the quantized embedding image $\bm{e}'$ and restore the original input images. Note that in actual implementations, $N$ input images are stacked along the channel dimension, with input channel size of $C = 3N$, denoted as $\{\bm{x}_c\}_{c=1}^C$ with $\bm{x}_c \in \mathbb{R}^{H \times W}$.

\textbf{Relation Module.} 
INNs have high architecture constraints, limiting their capacity of non-linear representation~\cite{dinh2015nice}. Thus, we propose a Relation Module to add some non-linear transformations while capturing cross-image relations. To prevent extra information loss in this stage, the transformation is performed at the same dimensional level with residual connections.

Details of the Relation Module are shown as the orange part in Figure~\ref{fig:overview}. $N$ parallel convolutional headers independently transform $N$ images into their feature space. The concatenation of the $N$ image features then goes through $N$ independent convolutional tailers plus residual connections to obtain the corresponding images with relational information extracted. The convolutional blocks used here are based on the Dense Block~\cite{Huang2017DBNet}. We can express the forward process of $f^i_{rel}$ for the $i^{th}$ image $\{\bm{x}_c\}_{c=3i-2}^{3i}$ as follows:
\begin{equation}
    \{\bm{r}_c\}_{c=3i-2}^{3i} = f^i_{rel}(\{\bm{x}_c\}_{c=1}^C) + \{\bm{x}_c\}_{c=3i-2}^{3i}.
\end{equation}
We then concatenate all $\{\bm{r}^i_c\}_{c=1}^{3}$ to obtain $\{\bm{r}_c\}_{c=1}^{C}$, with $\bm{r}_c \in \mathbb{R}^{H \times W}$. For the inverse process, we apply a symmetric Relation Module.

\textbf{Invertible Downscaling Module.} If we optionally activate the Invertible Downscaling Module, IICNet can embed the input images into a lower-resolution embedding image. This module is composed of either a Pixel Shuffling Layer (squeezing operation)~\cite{dinh2017density} or a Haar Wavelet Transformation Layer~\cite{viola2001rapid}, followed by an Invertible $1 \times 1$ Convolution~\cite{NEURIPS2018_d139db6a}. This module offers an invertible operation to halve the resolution of the input images, transforming the size of input tensor from $\mathbb{R}^{C \times H \times W}$ to $\mathbb{R}^{4C \times \frac{1}{2}H \times \frac{1}{2}W}$. The forward process of this module $f_{down}$ can be described as:
\begin{equation}
    \{\bm{u}_c\}_{c=1}^{C'} = f_{down}(\{\bm{r}_c\}_{c=1}^C),
\end{equation}
where $(C', W', H') = (4C, \frac{1}{2}H, \frac{1}{2}W)$, with $\bm{u}_c \in \mathbb{R}^{H' \times W'}$. If downscaling is disabled, $f_{down}$ is simply an identical function, yielding $\{\bm{u}_c\}_{c=1}^{C'} = \{\bm{r}_c\}_{c=1}^C$.

\textbf{Coupling Layers.} Following the design proposed in~\cite{ardizzone2018analyzing,dinh2015nice,dinh2017density}, we structure a deep INN architecture with several basic inveritble building blocks using two complementary affine coupling layers each. Considering the $i^{th}$ block, the $i^{th}$ input tensor $\{\bm{u}^i_c\}_{c=1}^{C'}$ is split into top (reference) parts $\bm{u}^i_t = \{\bm{u}^i_c\}_{c=1}^{c'}$ and bottom (non-reference) parts $\bm{u}^i_b = \{\bm{u}^i_c\}_{c=c'+1}^{C'}$ at position $c'$. The two corresponding affine transformations are formulated as follows, with element-wise multiplication $\odot$, exponential function $\text{exp}(\cdot)$, and centered sigmoid function $\sigma_c(\cdot) = 2\sigma(\cdot) - 1$:
\begin{equation}
    \bm{u}^{i+1}_t = \bm{u}^i_t + h_2(\bm{u}^i_b),
\end{equation}
\begin{equation}
    \bm{u}^{i+1}_b = \bm{u}^i_b \odot \text{exp}(\sigma_c(g(\bm{u}^{i+1}_t))) + h_1(\bm{u}^{i+1}_t),
\end{equation}
where the output tensor $\{\bm{u}^{i+1}_c\}_{c=1}^{C'} = [\bm{u}^{i+1}_t\ \bm{u}^{i+1}_b]$. We can then show that the two transformations are invertible:
\begin{equation}
    \bm{u}^{i}_b = (\bm{u}^{i+1}_b - h_1(\bm{u}^{i+1}_t)) \odot \text{exp}(-\sigma_c(g_1(\bm{u}^{i+1}_t))),
\end{equation}
\begin{equation}
    \bm{u}^{i}_t = \bm{u}^{i+1}_t - h_2(\bm{u}^i_b).
\end{equation}
Letting $f_{inn}$ be the forward pass of our INN architecture, the output tensor $\{\bm{v}_c\}_{c=1}^{C'}$ can be formulated as follows:
\begin{equation}
    \{\bm{v}_c\}_{c=1}^{C'} = f_{inn}(\{\bm{u}_c\}_{c=1}^{C'}).
\end{equation}

\begin{figure}[t]
\centering
    \includegraphics[width=1.0\linewidth]{figures/cs.pdf}
	\caption{Illustration of Channel Squeeze Layer}
	\label{fig:model_cs}
\end{figure}

\textbf{Channel Squeeze Layer.} We then need to reduce the channel dimension to obtain the embedding image $\bm{e}$. For the forward pass, the Channel Squeeze Layer treats its input tensor $\{\bm{v}_c\}_{c=1}^{C'}$ as a stack of preliminary RGB embedding images $\{\bm{e_n}\}_{n=1}^N$, and the embedding image $\bm{e}$ is calculated by averaging the preliminary embedding images:
\begin{equation}
    \bm{e} = f_{cs}(\{\bm{v}_c\}_{c=1}^{C'}) = average(\{\bm{e_n}\}_{n=1}^N).
\end{equation}
While for the backward pass, the Channel Squeeze Layer copies the quantized embedding image $\bm{\hat{e}}$ multiple times as $\{\bm{\hat{e}_n}\}_{n=1}^N$ and concatenates them along the channel dimension to match the channel size. 

Note that our network is jointly trained as a whole with inherent inverse functions of INNs, and the inverse pass takes the copied (same) quantized embedding images $\{\bm{\hat{e}_n}\}_{n=1}^N$ as input. This implicitly guides the embedding image $\bm{e}$ and all the preliminary embedding images $\{\bm{e_n}\}_{n=1}^N$ to look similar to each other. Hence, only minor noise is introduced to the invertibility, and there is no need to pose any explicit constraints on $\{\bm{e_n}\}_{n=1}^N$ during the forward pass. Figure~\ref{fig:model_cs} shows some visual patches of the preliminary embedding images during training, where all the preliminary embedding images are similar to each other. 
Also, we find that such implicit guidance on the preliminary embedding images helps stabilize the overall training process.
In fact, we have conducted some experiments to pose an explicit constraint between $\{\bm{e_n}\}_{n=1}^N$ and $\bm{e}$ or to use simple CNNs to model the information loss when reducing the channel dimension, but such designs make training unstable and achieve worse performance. 

\begin{table*}[t]
  \begin{center}
    \begin{tabular}{p{40pt}|p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}}
      \toprule[1pt]
      \multirow{3}{40pt}{\centering\textbf{Step}} & \multicolumn{4}{c}{\textbf{Embedding}} & \multicolumn{4}{c}{\textbf{Restored}} \\
      \ & \multicolumn{2}{c}{Zhu et al.~\cite{zhu-2020-video}} & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{Zhu et al.~\cite{zhu-2020-video}} & \multicolumn{2}{c}{Ours} \\
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 1 & \hfil 25.277 & \hfil 0.5608 & \hfil \textbf{37.750} & \hfil \textbf{0.9419} & \hfil 34.356 & \hfil 0.9363 & \hfil \textbf{36.866} & \hfil \textbf{0.9532} \\
      \hfil 3 & \hfil 24.561 & \hfil 0.5214 & \hfil \textbf{36.910} & \hfil \textbf{0.9245} & \hfil 33.099 & \hfil 0.9227 & \hfil \textbf{36.628} & \hfil \textbf{0.9502} \\
      \hfil 5 & \hfil 24.246 & \hfil 0.5056 & \hfil \textbf{36.576} & \hfil \textbf{0.9175} & \hfil 32.608 & \hfil 0.9170 & \hfil \textbf{36.462} & \hfil \textbf{0.9487} \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Comparison on Temporal Video Embedding test set with embeding range of $9$ and time step of $1$. }
  \label{tab:task1-comparison}
\end{table*}

\textbf{Quantization Layer.}
A quantization loss is unavoidable when one save the embedding image in common PNG format with only 8 bits per pixel per channel. There are many proposed methods like~\cite{Johannes2017End,theis2017lossy,Bengio2013EstimatingOP} to address this problem. In this paper, we choose to employ the method in~\cite{DBLP:journals/corr/BalleLS16a} to add uniform noise during training and do integer rounding during testing to obtain the quantized embedding image $\bm{\hat{e}}$.

\textbf{Inverse Process.} To restore the original input images, we can load the quantized embedding image $\bm{\hat{e}}$ and let it sequentially go through the inverse pass of IICNet:
\begin{equation}
    \{\bm{\hat{x}}_c\}_{c=1}^C = (f'_{rel} \circ f^{-1}_{down} \circ f^{-1}_{inn} \circ f'_{cs})(\bm{\hat{e}}),
\end{equation}
where $f'_{rel}$, $f^{-1}_{down}$, $f^{-1}_{inn}$, $f'_{cs}$ are the inverse pass functions of the corresponding modules. Then we can obtain the stored RGB images $\{\bm{\hat{i}}_n\}_{n=1}^N$.

\subsection{Loss Functions}
As discussed before in the Channel Squeeze Layer, we only need to employ loss functions at the two ends: the embedding image and the restored images.

\textbf{Embedding Image.} We employ $L_2$ loss to guide the embedding image $\bm{e}$ to be visually like the reference image $\bm{e}_{ref}$. In the case of downscaling, we use Bilinear method to downsample the reference image:
\begin{equation}
    \mathcal{L}_{emb} = ||\bm{e}_{ref} - \bm{e}||^2_2.
\end{equation}

In our experiments, we find that with $L_2$ loss only, the embedding image usually contains many high-frequency patterns. Hence, we further apply Fast Fourier Transform (FFT)~\cite{Brigham1967FFT} on both the embedding image and the reference image to obtain their frequency domain and add a frequency loss $\mathcal{L}_{freq}$ in terms of $L_2$ distance:
\begin{equation}
    \mathcal{L}_{freq} = ||FFT(\bm{e}_{ref}) - FFT(\bm{e})||^2_2.
\end{equation}

\textbf{Restored Images.} The restored images $\{\bm{\hat{i}}_n\}_{n=1}^N$ should match the original ones $\{\bm{i}_n\}_{n=1}^N$, so we have another basic restored loss $\mathcal{L}_{res}$ to minimize the average $L_1$ distance among each pair of the restored and original image:
\begin{equation}
    \mathcal{L}_{res} = \frac{1}{N} \sum_{n=1}^{N} ||\bm{i}_n - \bm{\hat{i}}_n||_1.
\end{equation}

\textbf{Total Loss.} To sum up, our proposed IICNet is optimized by minimizing the compact loss $\mathcal{L}_{total}$, with corresponding weight factors $\lambda_1$, $\lambda_2$, $\lambda_3$:
\begin{equation}
    \mathcal{L}_{total} = \lambda_1 \mathcal{L}_{emb} + \lambda_2 \mathcal{L}_{freq} + \lambda_3 \mathcal{L}_{res}.
\end{equation}


==> IICNet_ A Generic Framework for Invertible Image Conversion Camera Ready/tex/relatedwork.tex <==
\subsection{Reversible Image Conversion}
Our work solves the embedding-and-restoration problem, which belongs to the category of Reversible Image Conversion (RIC). Xia et al.~\cite{xia-2018-invertible} first proposed to encode the original color information into a synthesized grayscale image, from which the color image can be decoded. Recently, Video Snapshot~\cite{zhu-2020-video} tries to embed a sequence of video frames into one image for single image motion expansion. Hu et al.~\cite{hu-2020-mononizing} further attempts to build an invertible transformation between binocular views and monocular views. Although these approaches perform well in their own tasks with different technical designs, none of them can be generalized to all the tasks above because of task-specific design. Furthermore, these methods are generally based on a joint-trained encoder-decoder framework with limited ability to handle information loss problems.

The reversible property is also explored in steganography, which aims to hide information within different information carriers like images, where concealing and recovering the hidden information can be viewed as a reversible task. Recently, several learning-based methods~\cite{46526, tancik2020stegastamp, Wang2019HidingGANHC, Wengrowski_2019_CVPR, Zhu_2018_ECCV} leverage the pair of encoder and decoder to hide information in images. For example, Baluja~\cite{46526} tries to hide an image in another of the same size. Still, these works have a limited hiding capacity with some evident artifacts. In this work, we mainly focus on RIC tasks related to the image carrier only.

\subsection{Invertible Neural Networks}
Invertible neural networks (INNs)~\cite{dinh2015nice,dinh2017density,NEURIPS2018_d139db6a} guarantee the invertibility property with a careful mathematical design of network architecture and several invertible operations. In general, the forward process of an INN architecture can learn a bijective mapping between a source domain $x$ to a target domain $y$, with the forward process $f_{\theta}(x) = y$ and the inverse process $f^{-1}_{\theta}(y) = x$. A tractable Jacobian is another great characteristic of INNs to compute the posterior probabilities explicitly for the bijective mapping.

INNs are widely used in some generative tasks. Normalizing Flow based methods~\cite{NormalizingFlow,rezende2015variational} with INNs map a complex distribution $x$ with INNs to a latent distribution $z$ (e.g., Gaussian), which are usually trained by minimizing the unsupervised negative log-likelihood loss. Recent works further investigate the application of INNs on different tasks, such as image conditional image super-resolution~\cite{lugmayr2020srflow}, image generation~\cite{Ardizzone2019GuidedIG, Winkler2019LearningLW}, point cloud generation~\cite{Pumarola_2020_CVPR}, and segmentation tasks~\cite{Winkler2019LearningLW}. Different from Normalizing Flow based methods, IRN~\cite{xiao2020invertible} maps a high-resolution image to a low-resolution image by utilizing additional latent output variables with a cross-entropy loss in the image rescaling task. They claim that this latent space captures some knowledge of the lost high-frequency information~\cite{Shannon1949Communication}.
However, the lost information is usually more complex with not only high-frequency information in RIC tasks, making IRN difficult to generalize to different RIC tasks.

==> tex/conclusion.tex <==
We present a generic framework IICNet for various Reversible Image Conversion (RIC) tasks. IICNet maintains a task-independent and highly invertible architecture based on invertible neural networks (INNs), which largely mitigates the information loss problem. Due to strict invertibility, INNs have limitations in terms of dimensional flexibility and non-linear representation capacity. Our proposed Relation Module and Channel Squeeze Layer can greatly alleviate such limitations and preserve the information-reserving ability of INNs, promisingly applicable to other INNs applications.
IICNet yields state-of-the-art performance on some studied RIC tasks, such as Spatial-Temporal Video Embedding and Mononizing Binocular Images. We also extend to some unexplored tasks and the stenography task to further show the generalization of our IICNet. We hope the generalization and high performance of the proposed framework could help in more practical applications.


==> tex/experiments.tex <==
\begin{figure}
    \begin{subfigure}{1.0\linewidth}
        \includegraphics[width=0.98\linewidth]{figures/video-embedding.pdf}
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{1.0\linewidth}
        \begin{subfigure}{0.495\linewidth}\hfil Zhu et al.~\cite{zhu-2020-video}\end{subfigure}
        \begin{subfigure}{0.495\linewidth}\hfil Ours\end{subfigure}
	\end{subfigure}
	\caption{Visual result comparisons on embedding images.}
	\label{fig:task1-embedding}
\end{figure}

\begin{figure*}
    \begin{subfigure}{0.02\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Zhu et al.~\cite{zhu-2020-video}}}} \\
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}} \\
        \parbox[][1.9cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{1\linewidth}
            \includegraphics[width=1\linewidth]{figures/video-restore.pdf}
        \end{subfigure}
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.02\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 1\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 3\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 5 (ref.)\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 7\end{subfigure}
        \begin{subfigure}{0.195\linewidth}\hfil Frame 9\end{subfigure}
    \end{subfigure}
    \caption{Visual result comparisons on restored frames.}
	\label{fig:task1-restore}
\end{figure*}

This section first reports experiments conducted on previously-studied RIC tasks in Section~\ref{spatial-temporal-video-embedding} and~\ref{mononizing-binocular-images}, followed by the results of some newly-explored tasks in Section~\ref{dual-view-images} and~\ref{composition-and-decomposition-images}. In Section~\ref{hiding-images-in-an-image}, we also try the steganography task of hiding several images in one cover image. Please check out our supplementary materials for experimental setting details.

\subsection{Spatial-Temporal Video Embedding}
\label{spatial-temporal-video-embedding}

Video Snapshot~\cite{zhu-2020-video} aims to embed a sequence of video frames into one embedding image with the same resolution, which can be converted back to the original video sequence. Our proposed IICNet not only performs better but can even extend to embed the video frames spatiotemporally into a lower-resolution embedding image. 

\textbf{Dataset and Processing.} We use the high-quality DAVIS $2017$ video dataset~\cite{Jordi2017DAVIS} in this task. We use the official TrainVal set plus half of the Test-Dev set as the train set, another half of the Test-Dev set as the validation set, and the Test-Challenge set as the test set. To make our model more robust on different motion levels of video inputs, for each video sample in the train set, we subsample all the possible video subsamples with a time step of $5$ between consecutive frames, where we select the middle frame as the reference image.

\textbf{Result Comparison.} We only report the comparison results on the test set with embedding range $N = 9$, since Video Snapshot~\cite{zhu-2020-video} only provides the pre-trained model for this level of embedding range. We study on the performance at different time step levels of $1$, $3$, $5$ to test models' capacity in handling large motions. Statistics in Table~\ref{tab:task1-comparison} shows that our method significantly outperforms the baseline method at all time step levels by a large margin. Without dependence on optical flow, our method has less performance drop as the time step grows. We also offer grayscale PSNR and SSIM comparison in our supplemental materials for reference.

Figure~\ref{fig:task1-embedding} and Figure~\ref{fig:task1-restore} show the visualization results of the embedding images and the restored frames, respectively. Evident artifacts are found in the results of the baseline method, especially for the embedding image. In contrast, our embedding and restored images contain very few artifacts, demonstrating the effectiveness of the employed INN architecture in RIC tasks.

\begin{table}
  \begin{center}
    \begin{tabular}{p{29pt}|p{39pt}p{35pt}p{39pt}p{35pt}}
      \toprule[1pt]
      \multirow{2}{29pt}{\centering\textbf{Range}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 5 & \hfil 39.033 & \hfil 0.9539 & \hfil 41.836 & \hfil 0.9810 \\
      \hfil 7 & \hfil 38.336 & \hfil 0.9463 & \hfil 39.010 & \hfil 0.9674 \\
      \hfil 9 & \hfil 37.750 & \hfil 0.9419 & \hfil 36.866 & \hfil 0.9532 \\
      \hline\Tstrut
      \hfil 3 ($\bm{\times}$2) & \hfil 37.763 & \hfil 0.9608 & \hfil 36.891 & \hfil 0.9547 \\
      \hfil 5 ($\bm{\times}$2) & \hfil 36.622 & \hfil 0.9482 & \hfil 34.272 & \hfil 0.9242 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Results on Spatial-Temporal Video Embedding test set with different embedding ranges and resolutions.}
  \label{tab:task1-range}
\end{table}

\textbf{Embedding Range.} To investigate the embedding capacity of our method, we conduct experiments using different embedding ranges ($5, 7, 9$ input images). Similarly, we subsample the training videos with a time step of $5$, and test at a time step level of $1$. Intuitively, more input images indicate a more challenging task, where there is more motion information to be embedded into the embedding image. From Table~\ref{tab:task1-range}, we can see that our method outperforms the previous method at all levels of the embedding range and has less performance drop as the embedding range increases. 

\begin{figure*}[ht!]
    \begin{subfigure}{0.02\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][3.7cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{L. Bino-View}}} \\
        \parbox[][3.7cm][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{R. Bino-View}}}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \includegraphics[width=1\linewidth]{figures/mono.pdf}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.02\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
        \begin{subfigure}{0.256\linewidth}\hfil GT\end{subfigure}
        \begin{subfigure}{0.372\linewidth}\hfil Hu et al.~\cite{hu-2020-mononizing}\end{subfigure}
        \begin{subfigure}{0.372\linewidth}\hfil Ours\end{subfigure}
    \end{subfigure}
	\caption{Visual comparison results of the restored Binocular Images. We show the zoomed-in patches with the corresponding error map aside. Note that we amplified the error maps by 10 times for better visualization.}
	\label{fig:task2-comparison}
\end{figure*}

\textbf{Spatial-Temporal Embedding.} We further show the experimental results of our method to embed the input video sequence spatially and temporally into a lower-resolution embedding image. To the best of our knowledge, no previous work can do the spatial-temporal embedding task. We report the results of embedding $N = 3, 5$ into a $2$ times lower resolution in Table~\ref{tab:task1-range}. They are both conducted with a time step of $5$ and $1$ for training and testing, respectively. We can see that even we compress the input frames up to $20$ times smaller, still the model can have a good preview image and restored frames.

\textbf{Ablation Studies.} To validate the effectiveness of the components in our network and the utilization of the frequency loss, we report some ablation studies with embedding range of $5$ and a time step of $1$ in Table~\ref{tab:ablation}. From the experiments, we find the frequency loss greatly contributes to the artifacts-free embedding. Also, the proposed non-linear Relation Module works well to integrate the cross-image relationship and boost the performance.

\begin{table}
  \begin{center}
    \begin{tabular}{p{58pt}|p{29pt}p{29pt}p{29pt}p{29pt}}
      \toprule[1pt]
      \multirow{2}{58pt}{\centering\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil Ours w/o Fre. & \hfil 33.063 & \hfil 0.858 & \hfil 41.841 & \hfil 0.982 \\
      \hfil Ours w/o Rel. & \hfil 38.617 & \hfil 0.952 & \hfil 40.386 & \hfil 0.976 \\
      \hfil Ours & \hfil 39.033 & \hfil 0.954 & \hfil 41.836 & \hfil 0.981 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Ablation studies of frequency loss and Relation Module.}
  \label{tab:ablation}
\end{table}

\begin{table}[h!]
  \begin{center}
    \begin{tabular}{p{20pt}|p{56pt}|p{56pt}|p{56pt}}
      \toprule[1pt]
      \multirow{2}{20pt}{\ } & \multicolumn{1}{c|}{\textbf{Mono-view}} & \multicolumn{1}{c|}{\textbf{L. Bino-view}} & \multicolumn{1}{c}{\textbf{R. Bino-view}} \\ 
    %   \cline{2-5} & \hfil Snapshot & \hfil Ours & \hfil Snapshot & \hfil Ours \\
      \ & \hfil PSNR \text{  } SSIM& \hfil PSNR \text{  } SSIM & \hfil PSNR \text{  } SSIM \\
      \hline\Tstrut
      \hfil \cite{46526} & \hfil 26.1\ \ \ \ \ \ 0.81 & \hfil -\ \ \ \ \ \ \ \ \ \ \ \ - & \hfil 27.9\ \ \ \ \ \ 0.88 \\
      \hfil \cite{xia-2018-invertible} & \hfil 28.0\ \ \ \ \ \ 0.89 & \hfil 28.7\ \ \ \ \ \ 0.92 & \hfil 30.7\ \ \ \ \ \ 0.92 \\
      \hfil \cite{hu-2020-mononizing}  & \hfil 37.8\ \ \ \ \ \ \textbf{0.97} & \hfil 38.3\ \ \ \ \ \ 0.99 & \hfil 37.3\ \ \ \ \ \ 0.98 \\
      \hfil Ours & \hfil \textbf{37.9}\ \ \ \ \ \ 0.96 & \hfil \textbf{44.8}\ \ \ \ \ \ \textbf{0.99} & \hfil \textbf{39.4}\ \ \ \ \ \ \textbf{0.99} \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Results on Mononizing Binocular Images test set.}
  \label{tab:task2-comparison}
\end{table}

\subsection{Mononizing Binocular Images}
\label{mononizing-binocular-images}
We also experiment on another studied Mononizing Binocular Images task~\cite{hu-2020-mononizing}, which aims to convert binocular images or videos into monocular ones with the stereo information implicitly encoded. In this way, monocular devices can cope with stereoscopic data, and the original stereo content can be restored when necessary. We demonstrate that our framework outperforms state-of-the-art methods. 

Same as~\cite{hu-2020-mononizing}, we train on Flickr1024 dataset~\cite{Flickr1024} with the official train and test splits. Quantitative results are shown in Table~\ref{tab:task2-comparison}. We achieve the best performance especially for the restored images, with improvement of $6.5$dB for the left-views and $2.1$dB for the right-views. Although Mono3D already achieves good performance, still we can see some structural artifacts like the street lamp and the electric tower in the zoomed-in restored patches, as shown in Figure~\ref{fig:task2-comparison}, while our method can restore nearly artifact-free binocular-views. Although we only train our network on image dataset, when applying to video in a per-frame manner, the results show strong temporal consistency. Some demos can be found in supplementary materials.

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_normal.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/gt_zoom.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_normal.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.33\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_DualView/our_zoom.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.32\linewidth}\hfil Embedding\end{subfigure}
        \begin{subfigure}{0.32\linewidth}\hfil Normal-View\end{subfigure}
        \begin{subfigure}{0.32\linewidth}\hfil Zoomed-View\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Embedding Dual-View Images.}
	\label{fig:application1-visual}
\end{figure}

\begin{table}
  \begin{center}
    \begin{tabular}{p{35pt}|p{50pt}p{50pt}p{50pt}}
      \toprule[1pt]
      \hfil \textbf{Modes} & \hfil \textbf{Embedding} & \hfil \textbf{Normal} & \hfil \textbf{Zoomed} \\
      \hline\Tstrut
      \hfil $\times$ 2 & \hfil 38.541 & \hfil 50.277 & \hfil 43.806  \\
      \hfil $\times$ 4 & \hfil 38.271 & \hfil 48.740 & \hfil 43.694  \\
      \hfil $\times$ 8 & \hfil 38.607 & \hfil 48.923 & \hfil 43.610  \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Embedding Dual-View Images.}
  \label{tab:application1-psnr}
\end{table}


\subsection{Embedding Dual-View Images}
\label{dual-view-images}
Dual-View Camera Mode is an advanced technology in the field of smartphone cameras, which is first available on HUAWEI P30 Pro~\cite{dual_view}. Users can record split-screen images or videos with the primary camera capturing normal-view images or videos on the left and the zoom lens capturing zoomed-view ($\times 4$) images or videos on the right. 

Similar to binocular images, not all devices support dual-view images, where our method can serve as a backward-compatible solution by embedding the dual-view images into one normal-view image. We train and test our method using pairs of zoomed-view ($\times 2$,$\times 4$,$\times 8$) and normal-view images generated from the DIV2K dataset~\cite{Agustsson_2017_CVPR_Workshops}, with normal-view images as reference images. Detailed settings can be found in the supplementary materials.

Quantitative results in Table~\ref{tab:application1-psnr} show that our method achieves great performance to embed dual-view images in terms of both PSNR and SSIM. We also show some visual results in Figure~\ref{fig:application1-visual}, where we can see that both the embedding and restored images are nearly perfect. 

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_fg.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/gt_bg.jpeg}
		\end{subfigure}
	\end{subfigure}
	\\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_embedding.jpeg}
    	\end{subfigure}%
    	\begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_compose.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_fg.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.25\linewidth}
			\includegraphics[width=0.985\linewidth]{Image_adobe/our_bg.jpeg}
    	\end{subfigure}%
    \end{subfigure}
    \\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.24\linewidth}\hfil Embedding\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Composed\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Foreground\end{subfigure}
        \begin{subfigure}{0.24\linewidth}\hfil Background\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Composition and Decomposition.}
	\label{fig:application2-visual}
\end{figure}

\begin{table}
  \begin{center}
    \begin{tabular}{p{27pt}|p{38pt}p{38pt}p{38pt}p{38pt}}
      \toprule[1pt]
      \hfil \textbf{Task} & \hfil \textbf{Embed.} & \hfil \textbf{Comp.} &  \hfil \textbf{Fg.} & \hfil \textbf{Bg.} \\
      \hline\Tstrut
      \hfil Adobe & \hfil 45.638 & \hfil 52.672 & \hfil 45.120 & \hfil 45.071 \\
      \hfil Real & \hfil 46.757 & \hfil 58.324 & \hfil - & \hfil 44.325  \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Composition and Decomposition.}
  \label{tab:application2-psnr}
\end{table}

\subsection{Composition and Decomposition}
\label{composition-and-decomposition-images}
Photoshop~\cite{photoshop} is a popular image editing software, where users can use multiple layers to perform tasks such as compositing multiple images into one. Usually, the composition process is not reversible, so we cannot recover the sheltered part of the background of the composed image. However, with our method, we can allow the ``composed image" to embed all the layer images. In this way, although we only store and transmit one ``composed image" as before, users can also get the original layers for further usage.

Since there is no publicly available dataset for composition and decomposition, we instead train and test our method on two Matting datasets: Adobe Deep Matting dataset~\cite{deep-image-matting} and Real Matting dataset~\cite{BMSengupta20}. Note that Real Matting dataset does not have ground truth for foreground. Details setting is available in supplementary materials.

Table~\ref{tab:application2-psnr} shows the quantitative performance of our method on the two datasets. We also include some visual results in Figure~\ref{fig:application2-visual}. We can see that our method performs well and is verified to be applicable to the task of composing and decomposing images.

\begin{figure}
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{GT}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame1.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame2.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame3.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame4.jpeg}
    	\end{subfigure}%
	    \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/gt_frame5.jpeg}
    	\end{subfigure}%
	\end{subfigure}
	\\
    \begin{subfigure}{0.035\linewidth}
        % \setlength{\fboxsep}{0pt}\fbox{}
        \parbox[][][c]{\linewidth}{\centering\raisebox{0in}{\rotatebox{90}{Ours}}}
    \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_embedding.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame1.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame2.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame3.jpeg}
    	\end{subfigure}%
        \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame4.jpeg}
    	\end{subfigure}%
	    \begin{subfigure}{0.166\linewidth}
			\includegraphics[width=0.98\linewidth]{Image_General/our_frame5.jpeg}
    	\end{subfigure}%
	\end{subfigure}
	\\[2pt]
    \begin{subfigure}{0.035\linewidth}\hfil \end{subfigure}
    \begin{subfigure}{0.965\linewidth}
        \begin{subfigure}{0.155\linewidth}\hfil Embed.\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Cover\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 1\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 2\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 3\end{subfigure}
        \begin{subfigure}{0.155\linewidth}\hfil Rev. 4\end{subfigure}
    \end{subfigure}
	\caption{A sample result of Hiding Images in Image}
	\label{fig:application3-visual}
\end{figure}

\begin{table}
  \begin{center}
    % \renewcommand\tabcolsep{5.0pt}
    \begin{tabular}{p{41pt}|p{33pt}p{33pt}p{33pt}p{33pt}}
      \toprule[1pt]
      \multirow{2}{41pt}{\centering\textbf{\#\ Embed.}} & \multicolumn{2}{c}{\textbf{Embedding}} & \multicolumn{2}{c}{\textbf{Restored}} \\ 
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 2 & \hfil 38.911 & \hfil 0.9482 & \hfil 49.384 & \hfil 0.9951 \\
      \hfil 3 & \hfil 37.320 & \hfil 0.9277 & \hfil 43.671 & \hfil 0.9854 \\
      \hfil 4 & \hfil 36.221 & \hfil 0.9115 & \hfil 39.802 & \hfil 0.9743 \\
      \hfil 5 & \hfil 36.110 & \hfil 0.9064 & \hfil 37.777 & \hfil 0.9629 \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{PSNR on Hiding Images in an Image.}
  \label{tab:application3-psnr-ssim}
\end{table}

\subsection{Hiding Images in an Image}
\label{hiding-images-in-an-image}
To show the generality of our proposed model, we try the hardest task to hide several unrelated images with our model, which can be viewed as a kind of stenography. We obtain general images from the Flicker 2W dataset~\cite{liu2020unified}. We conduct experiments to embed $2$, $3$, $4$, $5$ images into one image, and the numerical results are listed in Table~\ref{tab:application3-psnr-ssim}. From the results, we can see that our method achieves relatively good performance even when embedding $5$ images into one, demonstrating the strong generality of our method. From the visual results shown in Figure~\ref{fig:application3-visual}, despite the variety of colors and structures of the images, we can restore them with no viewable artifacts.






==> tex/introduction.tex <==
Visual media can be classified into different types, including live photos~\cite{live_photo}, binocular images or videos~\cite{hu-2020-mononizing}, and dual-view images or videos~\cite{dual_view}. On the one hand, specific devices or platforms are required to view this visual media content. For example, binocular content may only be applicable in 3D devices, so we may need to generate corresponding monocular content to make them compatible with common devices~\cite{hu-2020-mononizing}. Instead of simply dropping part of the original content, a better choice is to build a reversible transformation, where the embedding is compatible with most devices, and the original content can be restored when necessary. On the other hand, a reversible single embedding image can help save the cost of storage and transmission bandwidth. To address these challenges, several Reversible Image Conversion (RIC) tasks~\cite{hu-2020-mononizing,xia-2018-invertible,zhu-2020-video} have been studied, which establish reversible transformation between visual content and an embedding image. Some examples are shown in Figure~\ref{fig:front}.

RIC tasks are challenging since we often need to embed much richer information implicitly in one single image, which may lead to unavoidable information loss. Hence, one of the key objectives in RIC tasks is to mitigate such information loss. However, previous works~\cite{hu-2020-mononizing,xia-2018-invertible,zhu-2020-video} usually employ an encoder-decoder based framework, which learns the informative bottleneck representation but has limited ability to capture the lost information~\cite{wang2020modeling,xiao2020invertible}. For example, Video Snapshot~\cite{zhu-2020-video} embeds a video preview into a single image and restores the original content by cascaded encoders and decoders. Although they sacrifice the embedding quality to embed as much information as possible, the restored frames are still not highly accurate. Furthermore, with the rapid growth of media formats, there is an increasing interest in the RIC tasks. Although RIC tasks share the same embedding-restoration procedure and the goal of obtaining high-quality embedding and restored images, previous methods usually have task-specific designs, such as optical flow in Video Snapshot~\cite{zhu-2020-video} and hardly generalize to other types of visual content. It is desirable to develop a general framework so that a generic framework can be adapted to all types of RIC tasks.

Considering these aspects, we propose Invertible Image Conversion Net (IICNet) as a generic framework for RIC tasks. To alleviate the information loss problem, we utilize invertible neural networks (INNs)~\cite{dinh2015nice,dinh2017density} as a strictly invertible embedding module. A Channel Squeeze Layer is also proposed to be incorporated into INNs for dimensional reduction while only minor deviation is introduced to the invertible architecture. Furthermore, to solve the problem that INNs contain limited non-linear transformation capacity~\cite{dinh2015nice}, we design a Relation Module to strengthen the non-linear representation capability that captures cross-image relation, in which the same-resolution transformation and residual connection help avoid extra information loss. These two new modules increase the flexibility and capacity of our network while keeping the advantage of INNs for reversibility. With strong embedding capacity and generic modules, IICNet does not rely on any task-specific technique as prior work, which makes it possible to deal with different content types. We also allow lower-resolution embedding for higher compression rates.

Here, we give a concrete example for illustration, as shown in Figure~\ref{fig:front}(a). Given a sequence of video frames, our IICNet can embed the spatial-temporal information of the sequence into one lower-resolution image that is visually similar to the downsampled middle reference frame.  There are some promising applications. First, we may embed a short video clip or live photo in one image. Second, we can embed a high-resolution high-FPS video into a low-resolution low-FPS video. In this way, we can allow flexible adoptions for different devices and save storage. Other potential applications are shown in Figure~\ref{fig:front}(b-e), including mononizing binocular images or videos, embedding dual-view images or multi-layer images, and even the general image hiding steganography task.

We conduct extensive experiments on five RIC tasks, in which our method outperforms other state-of-the-art methods by a large margin on all the studied tasks. Also, an ablation study is conducted for network modules and loss functions. Some detailed information and demo results are included in the supplementary materials. All the source codes and pre-trained models will be publicly available on Github. Our contributions are summarized as follows:
\begin{itemize}
    \item We present the first generic framework IICNet with the INN architecture that achieves state-of-the-art performance on five RIC tasks. IICNet allows various types of multimedia content to suit different devices and saves storage and bandwidth. 

    \item We propose a novel Channel Squeeze Layer and Relation Module incorporated into INNs to improve model flexibility and capacity while keeping the strength of reversibility.%, which can be extended to other applications with INNs.
    
    \item We study five practical RIC tasks, including two newly-explored ones, which are embedding a dual-view image into a single-view one and the reversible conversion between multi-layer images and a single image.

\end{itemize}

\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.5]{figures/overview.pdf}
\end{center}
\caption{Overview of the proposed network.}
\label{fig:overview}
\end{figure*}


==> tex/method.tex <==
The proposed IICNet for general Reversible Image Conversion (RIC) tasks aims to encode a series of input images into one reversible image (embedding image), which can have either the same or lower resolution. The embedding image can be decoded back to the original inputs with the network backward passing. The key is to use invertible neural networks (INNs) to model such a bijective mapping. An overview of our generic framework is shown in Figure~\ref{fig:overview}. Specifically, IICNet sequentially contains a \textbf{Relation Module}, an \textbf{Invertible Embedding Module} (an optional Invertible Downscaling Module plus several Coupling Layers), a \textbf{Channel Squeeze Layer}, and a \textbf{Quantization Layer}.

\subsection{Model Formulation} \label{model-formulation}
Formally, the input of IICNet is a series of $N$ input RGB images $\{\bm{i}_n\}_{n=1}^N$ with $\bm{i}_n \in \mathbb{R}^{3 \times H \times W}$, where $H$ and $W$ are the height and width, respectively. IICNet can forwardly encode the input images into an embedding image $\bm{e} \in \mathbb{R}^{3 \times H' \times W'}$, with embedding height $H'$ and width $W'$, which is visually indistinguishable from the reference image $\bm{e}_{ref}$. IICNet can then backwardly decode the quantized embedding image $\bm{e}'$ and restore the original input images. Note that in actual implementations, $N$ input images are stacked along the channel dimension, with input channel size of $C = 3N$, denoted as $\{\bm{x}_c\}_{c=1}^C$ with $\bm{x}_c \in \mathbb{R}^{H \times W}$.

\textbf{Relation Module.} 
INNs have high architecture constraints, limiting their capacity of non-linear representation~\cite{dinh2015nice}. Thus, we propose a Relation Module to add some non-linear transformations while capturing cross-image relations. To prevent extra information loss in this stage, the transformation is performed at the same dimensional level with residual connections.

Details of the Relation Module are shown as the orange part in Figure~\ref{fig:overview}. $N$ parallel convolutional headers independently transform $N$ images into their feature space. The concatenation of the $N$ image features then goes through $N$ independent convolutional tailers plus residual connections to obtain the corresponding images with relational information extracted. The convolutional blocks used here are based on the Dense Block~\cite{Huang2017DBNet}. We can express the forward process of $f^i_{rel}$ for the $i^{th}$ image $\{\bm{x}_c\}_{c=3i-2}^{3i}$ as follows:
\begin{equation}
    \{\bm{r}_c\}_{c=3i-2}^{3i} = f^i_{rel}(\{\bm{x}_c\}_{c=1}^C) + \{\bm{x}_c\}_{c=3i-2}^{3i}.
\end{equation}
We then concatenate all $\{\bm{r}^i_c\}_{c=1}^{3}$ to obtain $\{\bm{r}_c\}_{c=1}^{C}$, with $\bm{r}_c \in \mathbb{R}^{H \times W}$. For the inverse process, we apply a symmetric Relation Module.

\textbf{Invertible Downscaling Module.} If we optionally activate the Invertible Downscaling Module, IICNet can embed the input images into a lower-resolution embedding image. This module is composed of either a Pixel Shuffling Layer (squeezing operation)~\cite{dinh2017density} or a Haar Wavelet Transformation Layer~\cite{viola2001rapid}, followed by an Invertible $1 \times 1$ Convolution~\cite{NEURIPS2018_d139db6a}. This module offers an invertible operation to halve the resolution of the input images, transforming the size of input tensor from $\mathbb{R}^{C \times H \times W}$ to $\mathbb{R}^{4C \times \frac{1}{2}H \times \frac{1}{2}W}$. The forward process of this module $f_{down}$ can be described as:
\begin{equation}
    \{\bm{u}_c\}_{c=1}^{C'} = f_{down}(\{\bm{r}_c\}_{c=1}^C),
\end{equation}
where $(C', W', H') = (4C, \frac{1}{2}H, \frac{1}{2}W)$, with $\bm{u}_c \in \mathbb{R}^{H' \times W'}$. If downscaling is disabled, $f_{down}$ is simply an identical function, yielding $\{\bm{u}_c\}_{c=1}^{C'} = \{\bm{r}_c\}_{c=1}^C$.

\textbf{Coupling Layers.} Following the design proposed in~\cite{ardizzone2018analyzing,dinh2015nice,dinh2017density}, we structure a deep INN architecture with several basic inveritble building blocks using two complementary affine coupling layers each. Considering the $i^{th}$ block, the $i^{th}$ input tensor $\{\bm{u}^i_c\}_{c=1}^{C'}$ is split into top (reference) parts $\bm{u}^i_t = \{\bm{u}^i_c\}_{c=1}^{c'}$ and bottom (non-reference) parts $\bm{u}^i_b = \{\bm{u}^i_c\}_{c=c'+1}^{C'}$ at position $c'$. The two corresponding affine transformations are formulated as follows, with element-wise multiplication $\odot$, exponential function $\text{exp}(\cdot)$, and centered sigmoid function $\sigma_c(\cdot) = 2\sigma(\cdot) - 1$:
\begin{equation}
    \bm{u}^{i+1}_t = \bm{u}^i_t + h_2(\bm{u}^i_b),
\end{equation}
\begin{equation}
    \bm{u}^{i+1}_b = \bm{u}^i_b \odot \text{exp}(\sigma_c(g(\bm{u}^{i+1}_t))) + h_1(\bm{u}^{i+1}_t),
\end{equation}
where the output tensor $\{\bm{u}^{i+1}_c\}_{c=1}^{C'} = [\bm{u}^{i+1}_t\ \bm{u}^{i+1}_b]$. We can then show that the two transformations are invertible:
\begin{equation}
    \bm{u}^{i}_b = (\bm{u}^{i+1}_b - h_1(\bm{u}^{i+1}_t)) \odot \text{exp}(-\sigma_c(g_1(\bm{u}^{i+1}_t))),
\end{equation}
\begin{equation}
    \bm{u}^{i}_t = \bm{u}^{i+1}_t - h_2(\bm{u}^i_b).
\end{equation}
Letting $f_{inn}$ be the forward pass of our INN architecture, the output tensor $\{\bm{v}_c\}_{c=1}^{C'}$ can be formulated as follows:
\begin{equation}
    \{\bm{v}_c\}_{c=1}^{C'} = f_{inn}(\{\bm{u}_c\}_{c=1}^{C'}).
\end{equation}

\begin{figure}[t]
\centering
    \includegraphics[width=1.0\linewidth]{figures/cs.pdf}
	\caption{Illustration of Channel Squeeze Layer}
	\label{fig:model_cs}
\end{figure}

\textbf{Channel Squeeze Layer.} We then need to reduce the channel dimension to obtain the embedding image $\bm{e}$. For the forward pass, the Channel Squeeze Layer treats its input tensor $\{\bm{v}_c\}_{c=1}^{C'}$ as a stack of preliminary RGB embedding images $\{\bm{e_n}\}_{n=1}^N$, and the embedding image $\bm{e}$ is calculated by averaging the preliminary embedding images:
\begin{equation}
    \bm{e} = f_{cs}(\{\bm{v}_c\}_{c=1}^{C'}) = average(\{\bm{e_n}\}_{n=1}^N).
\end{equation}
While for the backward pass, the Channel Squeeze Layer copies the quantized embedding image $\bm{\hat{e}}$ multiple times as $\{\bm{\hat{e}_n}\}_{n=1}^N$ and concatenates them along the channel dimension to match the channel size. 

Note that our network is jointly trained as a whole with inherent inverse functions of INNs, and the inverse pass takes the copied (same) quantized embedding images $\{\bm{\hat{e}_n}\}_{n=1}^N$ as input. This implicitly guides the embedding image $\bm{e}$ and all the preliminary embedding images $\{\bm{e_n}\}_{n=1}^N$ to look similar to each other. Hence, only minor noise is introduced to the invertibility, and there is no need to pose any explicit constraints on $\{\bm{e_n}\}_{n=1}^N$ during the forward pass. Figure~\ref{fig:model_cs} shows some visual patches of the preliminary embedding images during training, where all the preliminary embedding images are similar to each other. 
Also, we find that such implicit guidance on the preliminary embedding images helps stabilize the overall training process.
In fact, we have conducted some experiments to pose an explicit constraint between $\{\bm{e_n}\}_{n=1}^N$ and $\bm{e}$ or to use simple CNNs to model the information loss when reducing the channel dimension, but such designs make training unstable and achieve worse performance. 

\begin{table*}[t]
  \begin{center}
    \begin{tabular}{p{40pt}|p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}p{44pt}}
      \toprule[1pt]
      \multirow{3}{40pt}{\centering\textbf{Step}} & \multicolumn{4}{c}{\textbf{Embedding}} & \multicolumn{4}{c}{\textbf{Restored}} \\
      \ & \multicolumn{2}{c}{Zhu et al.~\cite{zhu-2020-video}} & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{Zhu et al.~\cite{zhu-2020-video}} & \multicolumn{2}{c}{Ours} \\
      \ & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM & \hfil PSNR & \hfil SSIM \\
      \hline\Tstrut
      \hfil 1 & \hfil 25.277 & \hfil 0.5608 & \hfil \textbf{37.750} & \hfil \textbf{0.9419} & \hfil 34.356 & \hfil 0.9363 & \hfil \textbf{36.866} & \hfil \textbf{0.9532} \\
      \hfil 3 & \hfil 24.561 & \hfil 0.5214 & \hfil \textbf{36.910} & \hfil \textbf{0.9245} & \hfil 33.099 & \hfil 0.9227 & \hfil \textbf{36.628} & \hfil \textbf{0.9502} \\
      \hfil 5 & \hfil 24.246 & \hfil 0.5056 & \hfil \textbf{36.576} & \hfil \textbf{0.9175} & \hfil 32.608 & \hfil 0.9170 & \hfil \textbf{36.462} & \hfil \textbf{0.9487} \\
      \bottomrule[1pt]
    \end{tabular}
  \end{center}
  \caption{Comparison on Temporal Video Embedding test set with embeding range of $9$ and time step of $1$. }
  \label{tab:task1-comparison}
\end{table*}

\textbf{Quantization Layer.}
A quantization loss is unavoidable when one save the embedding image in common PNG format with only 8 bits per pixel per channel. There are many proposed methods like~\cite{Johannes2017End,theis2017lossy,Bengio2013EstimatingOP} to address this problem. In this paper, we choose to employ the method in~\cite{DBLP:journals/corr/BalleLS16a} to add uniform noise during training and do integer rounding during testing to obtain the quantized embedding image $\bm{\hat{e}}$.

\textbf{Inverse Process.} To restore the original input images, we can load the quantized embedding image $\bm{\hat{e}}$ and let it sequentially go through the inverse pass of IICNet:
\begin{equation}
    \{\bm{\hat{x}}_c\}_{c=1}^C = (f'_{rel} \circ f^{-1}_{down} \circ f^{-1}_{inn} \circ f'_{cs})(\bm{\hat{e}}),
\end{equation}
where $f'_{rel}$, $f^{-1}_{down}$, $f^{-1}_{inn}$, $f'_{cs}$ are the inverse pass functions of the corresponding modules. Then we can obtain the stored RGB images $\{\bm{\hat{i}}_n\}_{n=1}^N$.

\subsection{Loss Functions}
As discussed before in the Channel Squeeze Layer, we only need to employ loss functions at the two ends: the embedding image and the restored images.

\textbf{Embedding Image.} We employ $L_2$ loss to guide the embedding image $\bm{e}$ to be visually like the reference image $\bm{e}_{ref}$. In the case of downscaling, we use Bilinear method to downsample the reference image:
\begin{equation}
    \mathcal{L}_{emb} = ||\bm{e}_{ref} - \bm{e}||^2_2.
\end{equation}

In our experiments, we find that with $L_2$ loss only, the embedding image usually contains many high-frequency patterns. Hence, we further apply Fast Fourier Transform (FFT)~\cite{Brigham1967FFT} on both the embedding image and the reference image to obtain their frequency domain and add a frequency loss $\mathcal{L}_{freq}$ in terms of $L_2$ distance:
\begin{equation}
    \mathcal{L}_{freq} = ||FFT(\bm{e}_{ref}) - FFT(\bm{e})||^2_2.
\end{equation}

\textbf{Restored Images.} The restored images $\{\bm{\hat{i}}_n\}_{n=1}^N$ should match the original ones $\{\bm{i}_n\}_{n=1}^N$, so we have another basic restored loss $\mathcal{L}_{res}$ to minimize the average $L_1$ distance among each pair of the restored and original image:
\begin{equation}
    \mathcal{L}_{res} = \frac{1}{N} \sum_{n=1}^{N} ||\bm{i}_n - \bm{\hat{i}}_n||_1.
\end{equation}

\textbf{Total Loss.} To sum up, our proposed IICNet is optimized by minimizing the compact loss $\mathcal{L}_{total}$, with corresponding weight factors $\lambda_1$, $\lambda_2$, $\lambda_3$:
\begin{equation}
    \mathcal{L}_{total} = \lambda_1 \mathcal{L}_{emb} + \lambda_2 \mathcal{L}_{freq} + \lambda_3 \mathcal{L}_{res}.
\end{equation}


==> tex/relatedwork.tex <==
\subsection{Reversible Image Conversion}
Our work solves the embedding-and-restoration problem, which belongs to the category of Reversible Image Conversion (RIC). Xia et al.~\cite{xia-2018-invertible} first proposed to encode the original color information into a synthesized grayscale image, from which the color image can be decoded. Recently, Video Snapshot~\cite{zhu-2020-video} tries to embed a sequence of video frames into one image for single image motion expansion. Hu et al.~\cite{hu-2020-mononizing} further attempts to build an invertible transformation between binocular views and monocular views. Although these approaches perform well in their own tasks with different technical designs, none of them can be generalized to all the tasks above because of task-specific design. Furthermore, these methods are generally based on a joint-trained encoder-decoder framework with limited ability to handle information loss problems.

The reversible property is also explored in steganography, which aims to hide information within different information carriers like images, where concealing and recovering the hidden information can be viewed as a reversible task. Recently, several learning-based methods~\cite{46526, tancik2020stegastamp, Wang2019HidingGANHC, Wengrowski_2019_CVPR, Zhu_2018_ECCV} leverage the pair of encoder and decoder to hide information in images. For example, Baluja~\cite{46526} tries to hide an image in another of the same size. Still, these works have a limited hiding capacity with some evident artifacts. In this work, we mainly focus on RIC tasks related to the image carrier only.

\subsection{Invertible Neural Networks}
Invertible neural networks (INNs)~\cite{dinh2015nice,dinh2017density,NEURIPS2018_d139db6a} guarantee the invertibility property with a careful mathematical design of network architecture and several invertible operations. In general, the forward process of an INN architecture can learn a bijective mapping between a source domain $x$ to a target domain $y$, with the forward process $f_{\theta}(x) = y$ and the inverse process $f^{-1}_{\theta}(y) = x$. A tractable Jacobian is another great characteristic of INNs to compute the posterior probabilities explicitly for the bijective mapping.

INNs are widely used in some generative tasks. Normalizing Flow based methods~\cite{NormalizingFlow,rezende2015variational} with INNs map a complex distribution $x$ with INNs to a latent distribution $z$ (e.g., Gaussian), which are usually trained by minimizing the unsupervised negative log-likelihood loss. Recent works further investigate the application of INNs on different tasks, such as image conditional image super-resolution~\cite{lugmayr2020srflow}, image generation~\cite{Ardizzone2019GuidedIG, Winkler2019LearningLW}, point cloud generation~\cite{Pumarola_2020_CVPR}, and segmentation tasks~\cite{Winkler2019LearningLW}. Different from Normalizing Flow based methods, IRN~\cite{xiao2020invertible} maps a high-resolution image to a low-resolution image by utilizing additional latent output variables with a cross-entropy loss in the image rescaling task. They claim that this latent space captures some knowledge of the lost high-frequency information~\cite{Shannon1949Communication}.
However, the lost information is usually more complex with not only high-frequency information in RIC tasks, making IRN difficult to generalize to different RIC tasks.
